Generalizing Critical Path Analysis on Mobile Traffic

Critical Path Analysis (CPA) studies the delivery of webpages to identify page resources, their interrelations, as well as their impact on the page loading latency. Despite CPA being a generic methodology, its mechanisms have been applied only to browsers and web traffic, but those do not directly apply to study generic mobile apps. Likewise, web browsing represents only a small fraction of the overall mobile traffic. In this paper, we take a first step towards filling this gap by exploring how CPA can be performed for generic mobile applications. We propose Mobile Critical Path Analysis (MCPA), a methodology based on passive and active network measurements that is applicable to a broad set of apps to expose a fine-grained view of their traffic dynamics. We validate MCPA on popular apps across different categories and usage scenarios. We show that MCPA can identify user interactions with mobile apps only based on traffic monitoring, and the relevant network activities that are bottlenecks. Overall, we observe that apps spend 60% of time and 84% of bytes on critical traffic on average, corresponding to +22% time and +13% bytes than what observed for browsing.

==> sections/abstract_gioacchino.tex <==
%Critical Path Analysis (CPA) is a consolidated methodology to study web browsing traffic.
%It allows to dissect web page object relationships, and their importance on measuring standard performance metrics such as the page load time (PLT).
%Existing tools exclusively support web browsing as critical path analysis is founded on metrics such as PLT (Page Load Time) or webpage structure, which lack a definition for generic mobile applications. 

Critical Path Analysis (CPA) studies the delivery of web pages to identify page resources, their interrelations, as well as their impact on the page loading latency. 
Despite its merits, CPA internal mechanisms have been defined only for browsers, which do not automatically apply to any mobile app. 
Likewise, web browsing represents only a small fraction of the overall mobile traffic. 
In this paper we take a first step towards recovering this gap proposing \tool, a methodology to analyze mobile apps critical path purely relying on passive network observations. \tool is applicable to a broad spectrum of apps to expose a fine-grained view of their traffic dynamics.
We validate \tool on popular apps for different categories and under different scenarios. We show that \tool accurately identifies user interactions with mobile apps, and detects for the relevant intervals those activities that are bottlenecks in the resource delivery. We observe mobile apps spend significantly more time on critical path than browsing (\ie 55\% versus 38\%), this time being mostly related to apps control logic traffic.


%studies the delivery of webpages to identify page resources, their interrelations, 




==> sections/conclusion.tex <==
\section{Conclusion and Discussion}
\label{sec:conclusion}
In this paper we presented \tool, a methodology that generalizes critical path analysis for mobile traffic. Differently from state of the art metrics which are based on capturing the rendering of app on the screen, our methodology is based on traffic monitoring only. Results show that passive measurements are sufficient to both split traffic with respect to users activity with more than 84\% accuracy, and define a delivery deadline directly related to performance. Using active measurements we can further expose the critical components in the traffic mix, for instance highlighting the importance of app-specific domains.
We believe that \tool can be useful to different stakeholders.
App developers can pinpoint overheads related to flows creation and investigate the impact of network level (\eg TCP/TLS handshake, TCP fast open~\cite{tcpfastCONEXT11}) and app-specific protocols and control logic optimizations. ISPs can assess the effectiveness of core components in their networks (\eg DNS resolvers and pre-fetching, proxies enforced via APN configuration~\cite{almeida2017}) in regards of specific apps. Finally, end-users can have an objective way to quantify apps performance.
A few challenges still remains. \tool currently requires \texttt{pcap} files and is written in python. This limits its deployment at scale, so we are investigating how to port the tool on-device by mean Android VPN APIs, and how to extend it to iOS. This would allow us to further assess its capabilities with a larger measurements campaign. Another limitation is the use of active experiments to identify flows on the critical path. However, once \tool will be integrated on device, we plan to explore crowd-sourcing, \ie gather measurements from different devices and users, and define a methodology to identify common patterns impacting performance in the same spirit of KLOTSKI~\cite{klotski} and WebGaze~\cite{webgaze2017}.


==> sections/critical-table.tex <==
\begin{table}[!t]
%\footnotesize
\tiny
\centering
\caption{Critical path traffic characteristics.} 
\label{tab:critical}
\afnote{what if we group TCP and TLS? because we miss QUIC (or perhaps is grouped with TCP)?}

\hspace{-0.6cm}
\begin{tabular}{
    r@{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r 
     @{\hspace{1pt}} r
     @{\hspace{1pt}} r
     @{\hspace{1pt}} r
     @{\hspace{1pt}}|
    }
\multicolumn{1}{c}{} &
\multicolumn{12}{c}{app-startup} 
\\
\hhline{~------------}
\multicolumn{1}{@{\hspace{0pt}}c@{\hspace{1pt}}}{} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{fl.} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{dom.} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{vol.[kB]} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{T[s]} &
\multicolumn{4}{|@{\hspace{0pt}}c@{\hspace{1pt}}|}{T break [\%]}
\\
%App         & all   & CP    & all  & CP              \%Dns & \%Tcp & \%Tls/QUIC & \%Data \\ \hline
%Letgo       & 736   & 715   & 3.6  & 0.65            & 6     & 6     & 25         & 63     \\ \hline
%Amazon      & 1560  & 1490  & 8.22 & 6.98            & 0.4   & 7.8   & 22.8       & 69     \\ \hline
%CNN         & 80    & 25    & 7.06 & 2.69            & 15    & 15.8  & 3.8        & 65     \\ \hline
%Gmaps       & 880   & 870   & 7.3  & 4.2              & 0     & 12    & 25         & 63     \\ \hline
%Youtube     & 151   & 127   & 6.59 & 3.03            & 5.8   & 9     & 16         & 68.7   \\ \hline
%Outlook     & 22    & 20    & 2.7  & 2.15             & 3     & 10    & 22         & 65     \\ \hline
%NewsBreak   & 165   & 152   & 7.1  & 4.5              & 0     & 8     & 12         & 80     \\ \hline
%SoundCloud  & 726   & 715   & 10.6 & 8.15            & 0     & 6     & 16         & 78     \\ \hline
%Spotify     & 82    & 78    & 7.8  & 4.6              & 22    & 9     & 6          & 62     \\ \hline
%Uber        & 245   & 61    & 8.3  & 5.36            & 0     & 8     & 20         & 72     \\ \hline
%BBC         & 102   & 98    & 2.46 & 0.52            & 0     & 29    & 0          & 71     \\ \hline
             &abs  &\%   & abs &\%   &  abs   &\%    &abs  &\%    & DNS   & TCP   & TLS        & Data \\
\hhline{~------------}
%Letgo        &18   &30.0 & 10  &55.6 &  715   &97.1  &0.65 &18.1  & 6     & 6     & 25         & 63     \\ 
%Amazon       &49   &45.5 & 33  &67.3 &  1490  &95.5  &6.98 &84.9  & 0.4   & 7.8   & 22.8       & 69     \\ 
%CNN          &17   &12.5 & 10  &58.8 &  25    &31.3  &2.69 &38.1  & 15    & 15.8  & 3.8        & 65.4     \\
%Gmaps        &26   &46.2 & 17  &65.4 &  870   &98.9  &4.2  &57.5  & 0     & 12    & 25         & 63     \\
%Youtube      &16   &45.5 & 10  &62.5 &  127   &84.1  &3.03 &46.0  & 5.8   & 9     & 16         & 69.2   \\
%Outlook      &7    &50.0 & 4   &57.1 &  20    &90.9  &2.15 &79.6  & 3     & 10    & 22         & 65     \\
%NewsBreak    &41   &25.0 & 27  &65.9 &  152   &92.1  &4.5  &63.4  & 0     & 8     & 12         & 80     \\
%SoundCloud   &23   &20.0 & 10  &43.5 &  715   &98.5  &8.15 &76.9  & 0     & 6     & 16         & 78     \\
%Spotify      &8    &25.0 & 1   &12.5 &  78    &95.1  &4.6  &59.0  & 22    & 9     & 6          & 63     \\
%Uber         &22   &35.7 & 13  &59.1 &  61    &24.9  &5.36 &64.6  & 0     & 8     & 20         & 72     \\
%BBC          &8    &50.0 & 6   &75.0 &  98    &96.1  &0.52 &21.1  & 0     & 29    & 0          & 71     \\
%Facebook     &6    &50.0 & 7   &57.1 &  836   &96.7  &9.4  &61.3  & 1.0   & 0.2   & 6.1        & 92.7   \\
%Messenger    &5    &40.0 & 5   &40.0 &  86    &72.4  &2.4  &63.2  & 0     & 12.5  & 19.3       & 68.2     \\
%Twitter      &8    &12.5 & 13  &38.5 &  33    &79.1  &4.0  &77.7  & 0     & 14    & 18         & 68     \\
%Snapchat     &8    &50.0 & 10  &80.0 &  2802  &90.5  &10.8 &70.9  & 3     & 4     & 19         & 74     \\
%Instagram    &8    &25.0 & 16  &56.2 &  1108  &97.0  &3.7  &80.2  & 0     & 0.2   & 11.4       & 88.4     \\
%Gmail        &5    &20.0 & 7   &14.3 &  16    &90.9  &1.7  &82.4  & 0     & 17.6  & 28.9       &  53.5     \\
%Whatsapp{\color{red}*}         
%             & 2   &100  &2    &100  &  4     &100   & 0.9 &100   & 9     & 6     & 0          & 85     \\
Twitter     &13  &38   &1  &13   &33    &79   &4   &77    &0    &14    &18    &68\\
Facebook    &7   &40   &2  &40   &836   &97   &9   &61    &1    &0.2   &6.1   &92.7\\
Instagram   &16  &56   &2  &25   &1108  &97   &4   &80    &0    &0.2   &11.4  &88.4\\
\hhline{~------------}
Whatsapp    &2   &100  &1  &100  &4     &100  &1   &100   &9    &6     &0     &85\\
Snapchat    &10  &80   &4  &50   &2802  &91   &11  &70    &3    &4     &19    &74\\
Messenger   &5   &57   &3  &50   &86    &72   &2   &63    &0    &12.5  &19.3  &68.2\\
\hhline{~------------}
CNN         &10  &59   &2  &13   &25    &31   &3   &38    &15   &15.8  &3.8   &65.4\\
BBC         &6   &75   &2  &50   &98    &96   &1   &21    &0    &29    &0     &71\\
NewsBreak   &27  &66   &5  &25   &152   &92   &5   &63    &0    &8     &12    &80\\
\hhline{~------------}
Gmaps       &17  &65   &6  &46   &870   &99   &4   &57    &0    &12    &25    &63\\
Uber        &13  &59   &5  &36   &61    &25   &5   &64    &0    &8     &20    &72\\
\hhline{~------------}
Letgo       &10  &56   &3  &30   &715   &97   &1   &18    &6    &6     &25    &63\\
Amazon      &33  &67   &5  &45   &1490  &96   &7   &84    &0.4  &7.8   &22.8  &69\\
\hhline{~------------}
Gmail       &7   &14   &1  &20   &16    &91   &2   &82    &0    &17.6  &28.9  &53.5\\
Outlook     &4   &57   &2  &50   &20    &91   &2   &79    &3    &10    &22    &65\\
\hhline{~------------}
Youtube     &10  &63   &5  &45   &127   &84   &3   &46    &5.8  &9     &16    &69.2\\
SoundCloud  &10  &43   &2  &20   &715   &99   &8   &76    &0    &6     &16    &78\\
Spotify     &1   &13   &2  &25   &78    &95   &5   &59    &1    &9     &6     &84\\
\hhline{~------------}
AVERAGE     &11  &56   &3  &38   &513   &85   &4   &64    &2.5  &9.7   &15.1  &72.7\\
\hhline{~============}
Browsing      &12   &48 &5   &37  &488   &71    &5.53     &38    &2.6    &5.5    &16       &76\\
\hhline{~------------}
\end{tabular}
\hspace{-1pt}
\begin{tabular}{
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r @{\hspace{1pt}} r @{\hspace{1pt}}
    |@{\hspace{0pt}} r 
     @{\hspace{1pt}} r
     @{\hspace{1pt}} r
     @{\hspace{1pt}} r
     @{\hspace{1pt}}|
    }
\multicolumn{11}{c}{app-click} 
\\
\hhline{------------}
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{fl.} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{dom.} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{vol.[kB]} &
\multicolumn{2}{|@{\hspace{0pt}}c@{\hspace{1pt}}}{T[s]} &
\multicolumn{4}{|@{\hspace{0pt}}c@{\hspace{1pt}}|}{T break [\%]}
\\
%App         & all   & CP    & all  & CP              \%Dns & \%Tcp & \%Tls/QUIC & \%Data \\ \hline
%Letgo       & 736   & 715   & 3.6  & 0.65            & 6     & 6     & 25         & 63     \\ \hline
%Amazon      & 1560  & 1490  & 8.22 & 6.98            & 0.4   & 7.8   & 22.8       & 69     \\ \hline
%CNN         & 80    & 25    & 7.06 & 2.69            & 15    & 15.8  & 3.8        & 65     \\ \hline
%Gmaps       & 880   & 870   & 7.3  & 4.2              & 0     & 12    & 25         & 63     \\ \hline
%Youtube     & 151   & 127   & 6.59 & 3.03            & 5.8   & 9     & 16         & 68.7   \\ \hline
%Outlook     & 22    & 20    & 2.7  & 2.15             & 3     & 10    & 22         & 65     \\ \hline
%NewsBreak   & 165   & 152   & 7.1  & 4.5              & 0     & 8     & 12         & 80     \\ \hline
%SoundCloud  & 726   & 715   & 10.6 & 8.15            & 0     & 6     & 16         & 78     \\ \hline
%Spotify     & 82    & 78    & 7.8  & 4.6              & 22    & 9     & 6          & 62     \\ \hline
%Uber        & 245   & 61    & 8.3  & 5.36            & 0     & 8     & 20         & 72     \\ \hline
%BBC         & 102   & 98    & 2.46 & 0.52            & 0     & 29    & 0          & 71     \\ \hline
 abs &\%   &abs  &\%   &  abs   &\%    &abs  &\%    & DNS   & TCP   & TLS        & Data \\
\hhline{------------}
%Letgo       &5    &(100.0) &2    &(100.0) & 65   & (100)       & 2.43 &(100) & 0     & 1     & 5          & 94     \\ %\hline
%Amazon      &21   &(34.4)  &11   &(36.4)  & 1650 & (92.2)      & 12.2 &(80.8)  & 0     & 3     & 3          & 94     \\ %\hline
%CNN         &3    &(25.0)  &5    &(40.0)  & 69   & (82.1)      & 1.48 &(55.2)  & 0     & 3     & 0          & 97     \\ %\hline
%Gmaps       &3    &(60.0)  &2    &(100.0) & 870  & (98.9)      & 1.8  &(52.9)  & 0     & 0     & 0          & 100    \\ %\hline
%Youtube     &5    &(45.5)  &5    &(20.0)  & 65   & (47.4)      & 0.5  &(31.3)  & 0     & 23    & 42         & 35     \\ %\hline
%Outlook     &5    &(83.3)  &4    &(75.0)  & 9    & (100)       & 0.44 &(35.5)  & 0     & 21    & 54         & 25     \\ %\hline
%NewsBreak   &19   &(43.2)  &9    &(77.8)  & 96   & (20.9)      & 3    &(73.2)  & 0     & 7     & 6          & 87     \\ %\hline
%SoundCloud  &1    &(16.7)  &3    &(33.3)  & 120  & (99.2)      & 0.54 &(44.6)  & 0     & 0     & 0          & 100    \\ %\hline
%Spotify     &3    &(30.0)  &2    &(50.0)  & 115  & (98.3)      & 0.25 &(52.1)  & 0     & 0     & 0          & 100    \\ %\hline
%Uber        &3    &(42.9)  &2    &(50.0)  & 13   & (11.8)      & 5.43 &(85.2)  & 0     & 0     & 0          & 100    \\ %\hline
%BBC         &4    &(36.4)  &3    &(66.7)  & 105  & (92.9)      & 0.53 &(67.9)  & 0     & 22    & 0          & 78     \\ %\hline
%
%Facebook     & 5 &(40.0)&4   &(50.0) &  1313   &(63.8)& 4.6 & (54.6)  & 5.9   & 10   & 0.10   & 84   \\
%Messenger     & 5 &(40.0)&3   &(66.7) &  20   &(79.7)& 9.9 & (35.5)  & 0   & 26   & 29   & 45     \\
%Twitter   & 8 &(12.5)&4   &(25.0) &  29   &(96.9)& 18.7 & (44.24)  & 0   & 0   & 0   & 100     \\
%Snapchat   & 9 &(22.0)&3   &(33.0) &  194   &(75.4)& 5.7 & (17.0)  & 43   & 25   & 0   & 32     \\
%Instagram      & 7 &(57.1)&2   &(50.0) &  1538   &(90.8)& 1.8 & (50.9)  & 0   & 0.0   & 0.0   & 100     \\
%Gmail         & 11 &(54.5)&5   &(40.0) &  38   &(75.6)& 10.6 & (21.6) & 0  & 18   & 37   & 45    \\
%Whatsapp{\color{red}*}          & 1   &(100.0)&1    &(100.0) &  1.9    &(100.0)& 0.95 & (100.0)  & 0     & 0   & 0        & 100     \\
1   &13   &1  &25   &29    &96   &19  &44   &0   &0   &0        &100 \\
2   &40   &2  &67   &1313  &63   &5   &54   &5   &10  &0.1      &84 \\
4   &57   &1  &50   &1538  &90   &2   &50   &0   &0   &0        &100 \\
\hhline{------------}                                            
1   &100  &1  &100  &1     &100  &1   &100  &0   &0   &0        &100 \\
2   &22   &1  &33   &194   &75   &6   &17   &2  &4  &3        &91 \\
3   &60   &2  &40   &20    &79   &10  &35   &0   &1  &1       &98 \\
\hhline{------------}                                            
3   &25   &2  &40   &69    &82   &1   &55   &0   &3   &0        &97 \\
4   &36   &2  &67   &105   &92   &1   &67   &0   &22  &0        &78 \\
19  &43   &7  &78   &96    &20   &3   &73   &0   &7   &6        &87 \\
\hhline{------------}                                            
3   &60   &2  &100  &870   &98   &2   &52   &0   &0   &0        &100 \\
3   &43   &1  &50   &13    &11   &5   &85   &0   &0   &0        &100 \\
\hhline{------------}                                            
5   &100  &2  &100  &65    &100  &2   &100  &0   &1   &5        &94 \\
21  &34   &4  &36   &1650  &92   &12  &80   &0   &3   &3        &94 \\
\hhline{------------}                                            
6   &55   &2  &40   &38    &75   &11  &21   &0   &3  &4       &93 \\
5   &83   &3  &75   &9     &100  &0   &35   &0   &21  &54       &25 \\
\hhline{------------}                                            
5   &45   &1  &20   &65    &47   &1   &31   &0   &23  &42       &35 \\
1   &17   &1  &33   &120   &99   &1   &44   &0   &0   &0        &100 \\
3   &30   &1  &50   &115   &98   &0   &52   &0   &0   &0        &100\\
\hhline{------------}                                            
5   &48   &2  &56   &351   &79   &4   &55   &0   &5   &7       &88\\
\hhline{------------}                                            
\multicolumn{11}{c}{\rule{0pt}{1em}}
\end{tabular}


%App                                #Domains  #Critical_domains  #Flows  #Critical_flows
%com.abtnprojects.ambatana          10        3                  18      10
%com.amazon.mShop.android.shopping  11        5                  49      33
%com.cnn.mobile.android.phone       16        2                  17      10
%com.google.android.apps.maps       13        6                  26      17
%com.google.android.youtube         11        5                  16      10
%com.microsoft.office.outlook       4         2                  7       4
%com.particlenews.newsbreak         20        5                  41      27
%com.soundcloud.android             10        2                  23      10
%com.spotify.music                  8         2                  8       1
%com.ubercab                        14        5                  22      13
%bbc.mobile.news.uk                 4         2                  8       6


%\vspace{10pt}
%
%\begin{tabular}{
%    l@{$\,$}
%    |@{$\,$} r @{$\,\,$} r @{$\,$}
%    |@{$\,$} r @{$\,\,$} r @{$\,$}
%    |@{$\,$} r @{$\,\,$} r @{$\,$}
%    |@{$\,$} r @{$\,\,$} r @{$\,$}
%    |@{$\,$} r 
%     @{$\,$} r
%     @{$\,$} r
%     @{$\,$} r
%    }
%\multicolumn{1}{@{$\,$}c@{$\,$}}{} &
%\multicolumn{2}{@{$\,$}c@{$\,$}}{Flows} &
%\multicolumn{2}{@{$\,$}c@{$\,$}}{FQDN} &
%\multicolumn{2}{@{$\,$}c@{$\,$}}{Vol. [kB]} &
%\multicolumn{2}{@{$\,$}c@{$\,$}}{Time [s]} &
%\multicolumn{4}{@{$\,$}c@{$\,$}}{Time Break [\%]}
%\\
%%Application & Crit. path volume (tot) & Crit. path time (tot) & Time breakdown: & \%Dns & \%Tcp & \%Tls/QUIC & \%Data \\ \hline
%%Letgo         & 65KB (65KB)           & 2.43 (2.43)           &                   & 0     & 1     & 5          & 94     \\ \hline
%%Amazon        & 1.65MB(1.79MB)        & 12.2 (15.1)           &                   & 0     & 3     & 3          & 94     \\ \hline
%%CNN           & 69KB (84KB)           & 1.48 (2.68)           &                   & 0     & 3     & 0          & 97     \\ \hline
%%Gmaps         & 870KB (880KB)         & 1.8 (3.4)             &                   & 0     & 0     & 0          & 100    \\ \hline
%%Youtube       & 65KB (137KB)          & 0.5 (1.6)             &                   & 0     & 23    & 42         & 35     \\ \hline
%%Outlook       & 9KB (9KB)             & 0.44(1.24)            &                   & 0     & 21    & 54         & 25     \\ \hline
%%NewsBreak     & 96KB (460KB)          & 3 (4.1)               &                   & 0     & 7     & 6          & 87     \\ \hline
%%SoundCloud    & 120KB (121KB)         & 0.54 (1.21)           &                   & 0     & 0     & 0          & 100    \\ \hline
%%Spotify       & 115 KB (117KB)        & 0.25 (0.48)           &                   & 0     & 0     & 0          & 100    \\ \hline
%%Uber          & 13 KB (110KB)         & 5.43 (6.37)           &                   & 0     & 0     & 0          & 100    \\ \hline
%%BBC           & 105KB (113KB)         & 0.53 (0.78)           &                   & 0     & 22    & 0          & 78     \\ \hline
%\hhline{=============}
%App         &abs  &(\%)    &abs &all   &  abs   & (\%) & abs  & (\%)  & DNS   & TCP   & TLS        & Data \\
%\hline                          
%Letgo       &5    &(100.0) &2    &(100.0) & 65   & (100)       & 2.43 &(100) & 0     & 1     & 5          & 94     \\ %\hline
%Amazon      &21   &(34.4)  &11   &(36.4)  & 1650 & (92.2)      & 12.2 &(80.8)  & 0     & 3     & 3          & 94     \\ %\hline
%CNN         &3    &(25.0)  &5    &(40.0)  & 69   & (82.1)      & 1.48 &(55.2)  & 0     & 3     & 0          & 97     \\ %\hline
%Gmaps       &3    &(60.0)  &2    &(100.0) & 870  & (98.9)      & 1.8  &(52.9)  & 0     & 0     & 0          & 100    \\ %\hline
%Youtube     &5    &(45.5)  &5    &(20.0)  & 65   & (47.4)      & 0.5  &(31.3)  & 0     & 23    & 42         & 35     \\ %\hline
%Outlook     &5    &(83.3)  &4    &(75.0)  & 9    & (100)       & 0.44 &(35.5)  & 0     & 21    & 54         & 25     \\ %\hline
%NewsBreak   &19   &(43.2)  &9    &(77.8)  & 96   & (20.9)      & 3    &(73.2)  & 0     & 7     & 6          & 87     \\ %\hline
%SoundCloud  &1    &(16.7)  &3    &(33.3)  & 120  & (99.2)      & 0.54 &(44.6)  & 0     & 0     & 0          & 100    \\ %\hline
%Spotify     &3    &(30.0)  &2    &(50.0)  & 115  & (98.3)      & 0.25 &(52.1)  & 0     & 0     & 0          & 100    \\ %\hline
%Uber        &3    &(42.9)  &2    &(50.0)  & 13   & (11.8)      & 5.43 &(85.2)  & 0     & 0     & 0          & 100    \\ %\hline
%BBC         &4    &(36.4)  &3    &(66.7)  & 105  & (92.9)      & 0.53 &(67.9)  & 0     & 22    & 0          & 78     \\ %\hline
%
%Facebook     & 5 &(40.0)&4   &(50.0) &  1313   &(63.8)& 4.6 & (54.6)  & 5.9   & 10   & 0.10   & 84   \\
%Messenger     & 5 &(40.0)&3   &(66.7) &  20   &(79.7)& 9.9 & (35.5)  & 0   & 26   & 29   & 45     \\
%Twitter   & 8 &(12.5)&4   &(25.0) &  29   &(96.9)& 18.7 & (44.24)  & 0   & 0   & 0   & 100     \\
%Snapchat   & 9 &(22.0)&3   &(33.0) &  194   &(75.4)& 5.7 & (17.0)  & 43   & 25   & 0   & 32     \\
%Instagram      & 7 &(57.1)&2   &(50.0) &  1538   &(90.8)& 1.8 & (50.9)  & 0   & 0.0   & 0.0   & 100     \\
%Gmail         & 11 &(54.5)&5   &(40.0) &  38   &(75.6)& 10.6 & (21.6) & 0  & 18   & 37   & 45    \\
%Whatsapp{\color{red}*}          & 1   &(100.0)&1    &(100.0) &  1.9    &(100.0)& 0.95 & (100.0)  & 0     & 0   & 0        & 100     \\
%
%\hline
%\it {\color{red}avg(Update!)}          &16.2 &(47.0) & 4.4 &(59.0) & 288.8 & (76.7)      & 2.6  &(61.7)  & 0     & 7.1   & 10         & 82.7 \\
%\hline
%\end{tabular}
\end{table}
























%App                                #Domains  #Critical_domains  #Flows  #Critical_flows
%com.abtnprojects.ambatana          &5       &5 &2         &2                  
%com.amazon.mShop.android.shopping  &61      &21&11        &4                  
%com.cnn.mobile.android.phone       &12      &3 &5         &2                  
%com.google.android.apps.maps       &5       &3 &2         &2                  
%com.google.android.youtube         &11      &5 &5         &1                  
%com.microsoft.office.outlook       &6       &5 &4         &3                  
%com.particlenews.newsbreak         &44      &19&9         &7                  
%com.soundcloud.android             &6       &1 &3         &1                  
%com.spotify.music                  &10      &3 &2         &1                  
%com.ubercab                        &7       &3 &2         &1                  
%bbc.mobile.news.uk                 &11      &4 &3         &2                  







==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


Web browsing has been at the core of Internet services since its early days. 
Significant attention has been devoted to define metrics~\cite{bocchi2016,aft,info3,navigation-timing-level2} and methodologies~\cite{aaltodoc,goelPAM16,info3,wprofNSDI} to unveil webpages content delivery dynamics, and systems to optimize content delivery~\cite{klotski,webgaze2017,webprophet,shandianNSDI16}. These efforts are justified to improve end-users quality of experience (QoE), while service providers are incentivized to optimize their systems as their revenues are linked to users QoE.\footnote{https://www.fastcompany.com/1825005/how-one-second-could-cost-amazon-16-billion-sales}
Within these works, Critical Path Analysis (CPA) studies the delivery of webpages to identify page resources, their interrelations, and their impact on the user experience. To this goal, CPA first identifies a delivery deadline capturing the user QoE. For instance, the most widely adopted metric is \emph{Page Load Time} (PLT), the time elapsed between a user clicking a URL and the browser triggering the \texttt{onLoad} event.
%\afnote{can we make this general, and say then that CPA has been mostly used for browsing?} DP--As agreed this paragraph is about browsing
Once the deadline is defined, CPA investigates how each object download, parsing, and rendering tasks can be a bottleneck for the overall webpage delivery~\cite{klotski,wprofNSDI,shandianNSDI16}.
%\afnote{I would rephrase this because we didn't introduce what is a deadline nor PLT.}

The role of browsing is however shifting, as it is not at the center of user activities on mobile devices anymore.
Recent reports~\cite{flurrymobile,smartinsights} show that users spend less than 10\% of their time browsing, and more than 35\% on apps different than Facebook, streaming, gaming, and instant messaging.
%In other words, users do not use the browsers to consume the majority of the content they are interested into.
Such a trend is challenging also ad platforms where browsing on mobile devices generates half the conversion rate of desktops~\cite{grafik,monetate}. 
This progressive change in user interests and usage patterns is creating a \emph{gap in the literature}, and CPA has not been investigated in the context of generic mobile apps. 
At high level, CPA is based on three requirements: i) define a delivery deadline capturing the user QoE; ii) characterize network activities and their relationships %interrelations in the delivery of application content items; 
iii) identify which activities impact the delivery deadline, thus users QoE.

%\afnote{First...Second...the two points are abruptely introduced in the discussion flow. Can we rearrange this?}
To address the first requirement we need to answer the questions: ``\emph{Is any of the performance metrics defined for web traffic suited as delivery deadline for generic mobile apps? If not, how can we define a more suitable metric?}''. The literature has proposed several delivery deadlines.
%A \emph{delivery deadline} quantify the time needed to download and display some content. 
Despite PLT is the commonly used metric, \emph{Above The Fold} (AFT)~\cite{aft} and \emph{Speed Index} (SI)~\cite{speedindex} are considered superior.
Both have been introduced by Google % to study web traffic on desktop devices, but since they 
and focus on rendering dynamics measured via a screen capture. % rather than content and application properties. %, they can be used to study generic mobile traffic. 
%They require to take a video screen record, and to carefully process it to reduce the impact of dynamic content (\eg roll ads, and banners). 
%In other words, 
Their costs is not negligible, %, nor specific to mobile traffic~\cite{eyeorg}, 
and confine their adoption only to properly instrumented devices. Trying to solve AFT/SI constraints, the research community has proposed a flourished set of alternatives (Yslow, Object Index, DOMLoad, etc.~\cite{bocchi2016}). As for PLT, these metrics are easier to compute than AFT/SI, but they are all web traffic specific. %as related to events triggered by browsers. 
Conversely, AFT and SI do not make assumptions on content or application internals, so they are applicable to study generic mobile apps. %, although we are not aware of any study proving this.
%\afnote{drop the following sentence, as it's explained in the related?} For instance, PLT measures the time elapsed between a user clicking a URL and the browser firing the \texttt{onLoad} event indicating that the page has been loaded, \ie the metric is available only for browsers, and subject to their implementation. Overall, the first question to address is \afnote{perhaps comment out the 2nd question? We do define our own metric, but not sure we really address this question, meaning is really better?}

%State of the art metrics and methodologies have been forged in the context of web browsing, but they do not necessarily apply to generic mobile traffic. This is due to two main factors. First, there is the need to define a \emph{delivery deadline} capturing how long it takes to obtain some content. The most popular example is the page load time (PLT), which measures the time elapsed between a user clicking a URL and the browser firing the \texttt{onLoad} event indicating that the page has been loaded. Given its mechanics, PLT exists only for browsers. 
%Furthermore, despite W3C effort to standardize events related to web page download~\cite{navigation-timing,navigation-timing-level2}, different browsers might have different implementations, and measurements might not reflect dynamic content loading. 
%A more generalized delivery deadline is the Speed Index (SI), which measures the average time at which the visible parts of the page are displayed~\cite{speedindex}. By focusing on the rendering process, SI is generic enough to be applied to services other than browsing, but it is an invasive technique as requires video screen recording, so it is not suitable to be deployed at-scale. Overall, the literature offers a flourished set of metrics (Yslow, Object Index, DOMLoad, etc.)~\cite{bocchi2016} but they all suffer from the lack of generalization, instrumentation complexity, or lack of monitoring scalability. Hence, the first challenge we identify is \emph{how can we define a delivery deadline that is generic enough and applicable to monitor generic mobile traffic?} %: at-scale for thousands of users?}.

 
To understand traffic dynamics, identifying the right metric is not enough. Indeed, within the boundaries of each delivery deadline, a second question to address is ``\emph{How to identify which flows carry critical content for the overall delivery, without knowing the properties of the content itself?}''.
For instance, when considering web traffic, CPA leverages a \emph{dependency graph} where nodes represent the content downloaded while edges map the interdependecies between objects and related activities (\eg parsing, script execution, rendering).
%By investigates how each object download affects both the related objects, as well as the delivery deadline (\eg PLT), CPA can indentify bottlenecks in a webpage delivery~\cite{klotski,wprofNSDI,shandianNSDI16}. 
%Notice however that, 
While extracting such graph can be trivial for webpages (\eg parsing webpages source code, or inspecting the document object model - DOM), there is no guarantee that mobile content is served in the form of a webpage. It is therefore not clear how different network activities can be identified and how to understand which ones impact the delivery deadline.
 % And, can we identify the relationships between different flows when considering generic mobile traffic?}

Finally, another critical question is: ``\emph{Where is CPA performed?}''. The common choice in the literature~\cite{qoedoctorIMC14,shandianNSDI16,appinsightOSDI12} is an in full control scenario (\eg rooted device, apps source code, operating system ``modding''). In this case we can obtain fine-grained info at the cost of limiting the study to a few apps and users. Conversely, in the interest of enabling at-scale studies, we aim to study how to reduce the amount of on-device instrumentation in favour of a more traffic measurements centric approach.
%In a world with zero-latency networks, everything experienced by the user is related to rendering, but this is far from nowadays mobile traffic networks. Indeed, a previous study found that 35-85\% of mobile apps latency is due to downloads. A methodology purely based on traffic analysis can be used both on-device and in-network, but considering mobile apps heterogeneity, it is unclear \emph{``How much we can extrapolate from network traffic regarding app dynamics and user engagement?''}

%\afnote{Last, a more subtle factor to consider is \emph{where} the analysis should be performed. CPA is commonly done ``hooking'' browsers internals~\cite{klotski,wprofNSDI}. This entails that i) analysis are done on-device and ii) in the absence of a measurements standard, developers are responsibile to define what to measure and how. %Although on-device analysis can legerage some context information (which app is running, how the user is interacting, etc.), 
%it is unrealistic to expect that all apps would follow a common measurement standard even assuming one exists (which is not the case). 
%Furthermore, we argue that CPA is not necessarily tailored for end-users, as only developers and MNOs can act on bottlenecks (if any).
%In other words, sticking to a on-device measurements solution is too rigid, while a trully generic CPA for mobile traffic should be capable to cope with both on-device and in-network traffic analysis, so that both developers and MNOs can leverage useful insights.
%As the traffic itself is only common treat to both parties, it brings us to ask \emph{how accurate can be a methodology purely based on traffic analysis to identify performance issues?}}

%In this paper we present \tool, a methodology that generalises CPA for mobile traffic. \tool %brings fine-grained visibility into any mobile app traffic, and further highlights which components are critical. To do so, the traffic is processed in three phases.
%processes traffic in three phases.
%First, the traffic aggregate is split into \emph{activity windows}, each (possibly) corresponding to different user interactions with an app. Second, within the activity windows, a download waterfall is constructed to capture traffic dynamics over time, different metrics related to L4 and L7 dynamics are collected, and a delivery deadline is established.
%Finally, within each waterfall we identify which activities impact performance.

In this paper we present our journey in answering the previous questions.
%\afnote{large scale?}.
%and to understand if there is a case in using network traffic to dissecting mobile apps dynamics. 
We introduce a methodology, namely \emph{Mobile Critical Path Analysis} (MCPA), which combines passive and active measurements and heuristics to: i) recognize user interactions with applications; ii) extract network activities and relevant delivery deadlines; iii) identify network traffic that is critical for performance.
To understand the effectiveness of \tool we follow the standard practice of using an instrumented device, and we dissect the traffic of 18 popular mobile apps. 
Results show that via passive measurements we can identify user engagement with more than 80\% accuracy (\cref{sec:intervals}). We can also define delivery deadlines at least as good as PLT for browsing, and with less than 1.3s of error with respect to AFT in 75\% of tests with other apps (\cref{sec:waterfall}). By means of active experiments, we can split traffic into ``phases'' likely related to apps logic. Overall, we find that apps spend 60\% of time and 84\% of bytes on critical traffic on average (\cref{sec:cpa}).
Results support the idea of a new class of tools based on network measurements that ease the study of mobile apps.
%\dpnote{Write results according to above and what we have.}
%Results show that passive measurements can identify user engagement with more than 84\% accuracy (\cref{sec:intervals}), and the delivery deadline deviate no more than XXX from AFT/SI/PLT (\cref{sec:waterfall}). \tool also finds that the average time spent on the critical path is 55\% for apps, but 38\% for web browsing. 
%\afnote{add examples for some apps when we have them}
%We observe this time is mostly related to application control logic.} 
\tool source code and experimental datasets are publicly available.\footnote{\small\tt\mbox{\url{https://github.com/finale80/mcpa}}}


==> sections/introduction_ale.tex <==
\section{Introduction}
\label{sec:introduction}
Since its early days, the Web has been at the foundation of the Internet. The progressive shift towards mobile device usage is however starting to change this status quo. 
%Recent studies for instance show that more than 50\% of the web page requests are generate from mobile devices~\cite{statista,stonetemple} 
According to recent reports~\cite{smartinsights, flurrymobile},
users spend less than 10\% of their time browsing, and more than 35\% on apps different than Facebook, streaming, gaming, and instant messaging.
\afchange{In other words, browsing is not the main activity for users when using mobile devices, which instead use a large variety of other apps.} 
The reduced effectiveness of mobile browsing is also underlined when considering \afchange{webpages ads conversion rates: mobile platforms have half the value than for desktop}~\cite{grafik,monetate}. 

This \afchange{progressive change in user interests and usage patterns} has created a gap in the literature. On the one hand, there is a flourished set of methodologies~\cite{wprofNSDI,aaltodoc,info3,goel17}, metrics~\cite{Bocchi:2016:MQE,info3,navigation-timing,aft}, protocols~\cite{erman_2013CONEXT,han2015,han2016,http2}, and systems~\cite{wang2016,webgaze2017,webprophet,klotski} to study and optimize web browsing. On the other hand, such efforts require to be contextualized in order to be used to study mobile traffic. The most prominent example is \afchange{the} \emph{critical path analysis}, \ie the study of web pages to identify objects inter-dependencies, and how they impact a web page loading time. \afchange{By studying the web page structure and how is rendered by the browser}~\cite{wprofNSDI}, and by defining a delivery deadline (\eg Page Load Time -- PLT, DOMLoad, Above The Fold -- AFT time) it is possible to dissect the dynamics of a web page download~\cite{navigation-timing,navigation-timing-level2}. Such dynamics are expected to be present also in mobile traffic, but they are unlikely triggered by browsers, nor are necessarily carried over HTTP(S). \afchange{Android offers an \texttt{ActivityManager}~\cite{android-activitymanage} which allows to register some of the action triggered when using an app, but this is limited to XXX}

As first step to recover this gap, in this paper we discuss \tool, a methodology that generalises critical path analysis for mobile traffic. We aim to study traffic of any mobile app by relying on passive observations.
Such generalization comes with three target objectives. 
First, we start by observing that mobile traffic is bursty in nature, hence it can be divided in \emph{activity windows}, each (possibly) corresponding to different user interactions with an app. Second, within the activity windows, we build the download waterfall, \ie network and application level flows with timing information, and define a delivery deadline and performance indicators purely based on byte evolution over time. Third, we identify which network activities are bottleneck within every activity interval, \ie which activities determines the delivery performance and impact our performance indicators. \afnote{we need to introduce our metrics, as they are contribution}

We validate our methodology on the most popular apps for different app categories. We show that \tool identifies user interactions with 80-90\% accuracy. Further, performance metrics based on bytes exchange evolution over time are highly correlated with state of the art QoE metrics based on visual information (\ie AFT, and SpeedIndex -- SI). Finally, critical path analysis reveals only a fraction of network flows (about 30\%) actually determines the delivery performance.
\afnote{we can probably say more about the traffic, and differences between apps}
\tool source code and our experimental datasets are publicly available\footnote{\url{https://www.dropbox.com/sh/rk853z5e49l1mjy/AADOvq19EQ05R5ZDK_Jt0w1Ya?dl=0}}.


%traffic dependencies and delivery performance by mean of only passive measurements. This allows the methodology to be independent from app specific rendering triggers (e.g., onLoad). Still, we compare the our measurements with XXX showing that XXX

%Among those, the most known and adopted is arguably the PLT - page load time, measuring the time the browser takes to load a page\footnote{XXX add Better explanation of the actual meaning}. The metric gets an even stronger meaning in the context of a \emph{waterfall plot}, which describes how content is delivered over time.  By studying downloads inter dependencies, and which are key to define the PLT, i.e., by dissecting the \emph{critical path}, one can identify the element of which act to improve performance. For instance, by speeding up the deliver of XX the PLT reduce of YY ~\cite{XXX}

%Such methodology can be applied only if the PLT, or an equivalent index, can be measured. In other words, critical path analysis has been applied only to web browsing. This is particular limiting when considering mobile traffic. In fact, despite the predominance of HTTP(S), the browser is arguably the most used mobile app. In this context, state of the art content delivery indexes lack of formal definition: \emph{what is the PLT for a generic mobile app?}

%In this paper we discuss a methodology to study the critical path for mobile traffic, defined to achieve to specific objectives. 



==> sections/metrics.tex <==
\section{Critical Path Analysis}
\label{sec:metrics}

%\dpnote{We need to describe existing metrics and non applicability in RW. See also comment below}

This section describe how \tool quantifies delivery performance of every activity interval, and it identifies network activities that are bottleneck for every interval. 

\subsection{Performance metric}
The goal of the performance metric is not to provide a precise quantification of the Quality of Experience perceived by users, but rather to provide a reference value over which analyzing the impact of different network activities. 
As discussed in Sec~\ref{sec:related}, previously proposed techniques to analyze browsing critical path rely on the PLT (Page Load Time) as reference metric. However, PLT is not defined in the context of a generic mobile application, and more generally there are not reference performance metrics measuring the loading time of a mobile app.

In absence of application layer information, our rationale is that a good indicator of performance is the evolution of the byte exchanged over time. 
Therefore, we define the \emph{Transport Delivery Time} (TDT), as the time between the beginning of an activity interval and the time at which 99\% of the total bytes exchanged in the interval are transferred. The choice of the 99th-percentile is driven by our experience with the analyzed applications where we observe 99\% of bytes are transferred in burst, while some bytes are further exchanged at slower peace, \eg keep alive, app reporting.

TDT, as a time instant metric similar to PLT, provides an indication of how long the user has to wait for the app to complete the action it requires. However, it does not capture what the quality of the download is within this interval. Therefore, we propose the \emph{Transport Delivery Index} (TDI) integral metric  to solve this issue:

\begin{equation}
TDI=\int_0^{TDT} (1-x_B(t)) dt
\end{equation}

where $x_B(t)$ is the percentage of bytes retrieved at time t.


\subsection{Identifying bottleneck activities}
To extract the critical path from the waterfall of an activity interval, it is essential detecting those activities that may significantly delay the resource delivery. In the case of web browsing, this can be achieved by instrumenting test pages or by explicitly injecting delays in open source browser engines such as Webkit. However, both methods are not applicable to the case of mobile apps. As such, \tool takes a different approach \gtnote{add reference to Webprophet}, which consists in shaping the traffic associated with each domain name in the activity interval, using the \textit{tc} traffic control tool on the test device, and analyzing the corresponding impact on the waterfall.
This analysis, whose result is the indication of the critical path, is performed in two steps. 

In the first one, \tool quantifies, for each domain under shaping, the corresponding effect on the performance metric (TDT) \gtnote{I would include AFT as well, but only in evaluation/validation}. The result is the set of {\it critical} domains, i.e. domains for which a delay in the download/data-exchange will affect the overall delivery performance. Flows belonging to such domains form the critical path for the interval/waterfall under analysis.
In the second step, \tool enriches the initial information by extracting the dependencies between domains operating in the relevant interval. Given two domains \textit{x} and \textit{y}, and being $T_x$ and $T_y$ the times at which downloads from \textit{x} and \textit{y} terminate, we say domain \textit{y} is dependent on domain \textit{x} if the increase of $T_x$, obtained through traffic shaping, have a clear effect on $T_y$.

For both steps, \tool needs to decide if the impact of traffic shaping performed on domain $x$ -- in the first case on TDT, in the second case on the download completion times $T_y$  of other domains \textit{y} -- is significant or not. However, the download times can also "naturally" fluctuate, thus generating uncertainty, due to changes in the network conditions as well as variations in the displayed application content, e.g. new images replacing old ones. 
To address this problem we perform multiple (at least 10) experiments for each activity interval and shaped domain, and we use p-value tests to validate or reject changes of the target time (TDT or any $T_y$) obtained when shaping domain \textit{x} (given how the target metric is distributed when no shaping occurs). \gtnote{probably I should keep only few details}. If, set the significance level to $0.05$, the null hypothesis  (i.e, "Shaping domain \textit{x} does not affect the target time") is rejected for every experiment, domain \textit{x} is flagged as \textit{critical}, or added as a dependency for domain \textit{y}.             
\dpnote{This plot is from imc poster}

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{fig/waterfall.png}
\caption{Waterfall for Outlook}
\label{fig:waterfall-example}
\end{figure}

As example, we can consider the network waterfall in Fig.~\ref{fig:waterfall-example}, which refers to Microsoft Outlook application at startup. In this case seven domain names participate to the waterfall: \url{app.adjust.com}. \url{by.uservoice.com}, \url{prod15-api.acompli.net}, \url{data.flurry.com}, \url{...}. Each of them is passed to the traffic shaper, and the TDT is evaluated over multiple experiments. From the analysis, only \url{prod15-api.acompli.net}   
and \url{prod15-files.acompli.net} are flagged as critical, as only in these two cases the resulting TDT leads, for every experiment, to a p-value below 0.05 (significance level). Running similar tests, but on the per-domain download  completion times instead of TDT, \tool finds  \url{prod15-api.acompli.net}  and \url{prod15-files.acompli.net} also depend each other, and no other dependency is detected. With such knowledge, \tool finally builds the critical path pointing, as in  Fig.~\ref{fig:waterfall-example}, at those flows belonging to critical domains. \gtnote{shall we keep same example, and change figure 1?}

\subsection{Evaluation and discussion}

In Fig.~\ref{fig:waterfall-example} we also report the critical path for Outlook at startup.


%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{fig/waterfall.png}
%\caption{Waterfall for Outlook}
%\label{fig:waterfall-example}
%\end{figure}


In this section we measure TDT and TDI for different applications on different scenarios by varying the network conditions, and analyze if they actually capture the quality of the application delivery and can thus be used as reference to identify the critical path. We also compare TDT and TDI to \emph{Above the Fold Time (AFT)} and \emph{SpeedIndex} to understand how much they are correlated to state-of-the-art metrics commonly used for web browsing.
%As highlighted in Sec~\ref{sec:related} those metrics are not suitable \dpnote{Definition of those metrics and limitations in RW, and report short summary here} but can be used as reference for comparison.

Fig.~\ref{fig:qoe-diff} reports the absolute difference between TDT and the baseline AFT normalized over AFT. We also report results obtained for regular browsing of top-100 Alexa websites as reference. \dpnote{Honestly I would remove}
We first observe the average ratio  
\dpnote{I would also add a plot about normalized difference between AFT e TDT}

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{fig/comparison_with_alexa.pdf}
\caption{Normalized difference {\bf TDT - AFT}}
\label{fig:qoe-diff}
\end{figure}

We then analyze the correlation among the different metric. \dpnote{Add table if it makes sense} \gtnote{I would keep only one table, with startup.after-startup all together}.

\begin{table}[t]
\centering
\caption{Correlation coefficients from Pearson correlation matrix. Case=mobile apps, all activities (startup, after startup), 4g}
\label{table1l}
\begin{tabular}{|l|l|l|l|l|}
\hline
            & TDT & AFT  & TDI  & Speed index \\ \hline
TDT         &     & 0.85 & 0.94 & 0.71        \\ \hline
AFT         &     &      & 0.79 & 0.80        \\ \hline
TDI         &     &      &      &             \\ \hline
Speed index &     &      & 0.71 &             \\ \hline
\end{tabular}
\end{table}

\dpnote{After presenting those results, discuss what are the reasons of the delta among the metrics and that there is not a clear correlation between bytes, app category and this delta}.


==> sections/metrics_gioacchino.tex <==
\section{Critical Path Analysis}
\label{sec:cpa}

The last step of \tool is the identification of the critical path of every activity window, \ie network flows that are bottleneck in the delivery of application resources. 
Our rationale is to first run every application multiple times, each time shaping the traffic associated to one domain name in the activity interval, using the \textit{tc} traffic control tool on the test device.
Then, we identify from those experiments which domains have an actual impact on the performance metric TDT. 
The result is the set of {\it critical} domains, i.e. domains for which a delay in the download/data-exchange will affect the overall delivery performance. Flows belonging to such domains constitute the critical path for the activity window under analysis.

To determine if a given domain $x$ is critical, \tool needs to determine if the impact of traffic shaping performed on domain $x$ 
is significant or not. However, TDT is not constant across experiments even without any traffic shaping, \eg  variable network conditions.
To address this problem we perform multiple experiments for each activity window and shaped domain, and we use p-value tests to validate or reject changes of the target time (TDT) with respect to the scenario without any traffic shaping.
We set the significance level to $0.05$, and if the null hypothesis  (\ie "Shaping domain \textit{x} does not affect the target time") is rejected for every experiment, domain \textit{x} is added to the list of critical domains.          
\dpnote{This plot is from imc poster}

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{fig/waterfall.png}
\caption{Waterfall for Outlook}
\label{fig:waterfall-example}
\end{figure}

\gtnote{missing: how to group segments/flows of critical domains to form the critical path}
\dpnote{fix this once new plot is ready}
As example, we can consider the network waterfall in Fig.~\ref{fig:waterfall-example}, which refers to Microsoft Outlook application at startup. In this case seven domain names participate to the waterfall: \url{app.adjust.com}. \url{by.uservoice.com}, \url{prod15-api.acompli.net}, \url{data.flurry.com}, \url{...}. Each of them is passed to the traffic shaper, and the TDT is evaluated over multiple experiments. From the analysis, only \url{prod15-api.acompli.net}   
and \url{prod15-files.acompli.net} are flagged as critical, as only in these two cases the resulting TDT leads, for every experiment, to a p-value below 0.05 (significance level). Running similar tests, but on the per-domain download  completion times instead of TDT, \tool finds  \url{prod15-api.acompli.net}  and \url{prod15-files.acompli.net} also depend each other, and no other dependency is detected. With such knowledge, \tool finally builds the critical path pointing, as in  Fig.~\ref{fig:waterfall-example}, at those flows belonging to critical domains. \gtnote{shall we keep same example, and change figure 1?}

\subsection{Evaluation and discussion}
In this section we first validate our critical path analysis methodology, then we report critical path properties for the applications we analyzed.
In absence of application layer information to identify the actual critical path, we use as as baseline the methodology described above by using as performance metric AFT.
%Here we validate the approach adopted by \tool to build the critical path for each user activity interval starting from the corresponding network waterfall. Our approach cannot be directly compared to state-of-the-art techniques, such as the ones in \gtnote{cite Wprof, ..}, as these rely on PLT metrics that are not exposed in the case of mobile applications. However, we can still validate our technique by looking at the impact of the critical path on the visualization, Therefore, as a reference we compute "ground-truth" critical paths based on the \emph{Above the Fold Time (AFT)}.... More conversely we perform, similarly to our technique, traffic shaping for each domain and we tag as critical those domains with a significant impact on AFT, instead of the TDT metric used by \tool. The resulting domain set is used to derive the baseline critical paths.
%To validate our approach, we first need to demonstrate that the critical domain sets extracted by \tool approximate well the ground-truth ones computed with the AFT. In addition, we evaluate whether \tool provides, with respect to the reference approach, similar indications in terms of download traffic volume on the critical path and their total duration.

We first look into the domains that are identified as critical in Table~\ref{tab:}. We

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{fig/cp_number_critical.pdf}
\caption{Critical domains with respect to baseline}
\label{fig:cp-comp}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{fig/cp_comparison_volume_time.pdf}
\caption{Increase of volume and duration wrt baseline}
\label{fig:cp-num}
\end{figure}     

Takaways from Fig.~\ref{fig:cp-comp} and Fig.~\ref{fig:cp-num}.. The set of critical domains extracted by \tool well approximates the reference ones obtained using AFT. In particolar, all domains marked as critical in the baseline approach, will also be considered by \tool for building the critical path. For some applications, \tool will also include domain names that do not significantly impact the AFT. However, we can in Fig.~\ref{fig:cp-num}  that the critical path found by \tool exhibit similar characteristics compared to the baseline ones, both in terms of total download size and of duration \gtnote{need to come back on this, as it may sound redundant}.     

\textbf{Properties of critical path}
We first evaluate the impact of critical path 
\begin{figure}
\centering
\subfigure[]{
  \centering
  \includegraphics[width=.45\linewidth]{fig/cp_startup.pdf}
%  \caption{Application startup}
  \label{fig:cp_sub1}
 }
\subfigure[]{
  \centering
  \includegraphics[width=.45\linewidth]{fig/cp_after_startup.pdf}
%  \caption{Application usage (after startup)}
  \label{fig:cp_sub2}
  }
\caption{General properties of critical path (a=startup, b=after startup)}
\label{fig:cp}
\end{figure}



    



==> sections/screenrec.tex <==
\subsection{Impact of screen recording}
\label{screenrec}
As the video screen record can be resource demanding, it can bias the measurement of AFT and SI, as well as our defined deadline TDT and TDI.
To investigate on this, we consider the apps startup, and run 10 experiments for each app with and without \texttt{Android screenrecord} enabled. For each experiment we collect two metrics: TDT over the app startup activity window, and %which is used to evaluate whether the screen record slows the byte exchange down. The second metric is the 
the \texttt{Displayed} time\footnote{\url{https://developer.android.com/topic/performance/vitals/launch-time}} provided by \texttt{Android Activity Manager}\footnote{\url{https://developer.android.com/reference/android/app/ActivityManager}} via \texttt{logcat} for those activities involved in the app startup (\eg launching the process, initializing the objects, creating the activity, inflating the layout, and drawing the application for the first time). In other words, we are interested in understanding if (and by how much) these deadline changes in the presence of the screen record with respect to the bytes exchanged, as well as the dynamics of the apps.

\begin{figure*}[!t]
\centering
\includegraphics[width=0.51\textwidth]{fig/screenrec_tdt.pdf}
\includegraphics[width=0.47\textwidth]{fig/screenrec_displayed.pdf}
\caption{Impact of screen recording. \label{fig:screenrec}}
%\afnote{TODO: add final results} \gtnote{we have now 40/50 website}
\end{figure*}

In Fig~\ref{fig:screenrec} we compare the median TDT (left) and Displayed times (right) across apps and experiments. Notice how the points are well distributed over the bisect line, with only two corner cases for the Display time (Uber and Whatsapp). With an error generally lower than 1\%, we can conclude that for the apps under study the impact of the screen record is marginal.

